A Design-Time/Run-Time Application Mapping Methodology for Predictable Execution Time in MPSoCs

Executing multiple applications on a single MPSoC brings the major challenge of satisfying multiple quality requirements regarding real-time, energy, etc. Hybrid application mapping denotes the combination of design-time analysis with run-time application mapping. In this article, we present such a methodology, which comprises a design space exploration coupled with a formal performance analysis. This results in several resource reservation configurations, optimized for multiple objectives, with verified real-time guarantees for each individual application. The Pareto-optimal configurations are handed over to run-time management which searches for a suitable mapping according to this information. To provide any real-time guarantees, the performance analysis needs to be composable and the influence of the applications on each other has to be bounded. We achieve this either by spatial or a novel temporal isolation for tasks and by exploiting composable NoCs. With the proposed temporal isolation, tasks of different applications can be mapped to the same resource while with spatial isolation, one computing resource can be exclusively used by only one application. The experiments reveal that the success rate in finding feasible application mappings can be increased by the proposed temporal isolation by up to 30% and energy consumption can be reduced compared to spatial isolation.

==> acropatch.tex <==
% Extend acronym package with first letter caps
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
  \ifcsname fn@#1@PL\endcsname%
    \ifAC@uppercase@first%
      \expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
    \else%
      \csname fn@#1@PL\endcsname%
    \fi%
  \else%
    \AC@acl{#1}s%
  \fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
  \ifcsname fn@#1@PL\endcsname%
    \ifAC@uppercase@first%
      \expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
    \else%
      \csname fn@#1@PL\endcsname%
    \fi%
  \else%
    \AC@ac{#1}s%
  \fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
  \ifcsname fn@#1@PL\endcsname%
    \ifAC@uppercase@first%
      \expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
    \else%
      \csname fn@#1@PL\endcsname%
    \fi%
  \else%
    \AC@acf{#1}s%
  \fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
  \ifcsname fn@#1@PL\endcsname%
    \ifAC@uppercase@first%
      \expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
    \else%
      \csname fn@#1@PL\endcsname%
    \fi%
  \else%
    \AC@acs{#1}s%
  \fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
  \@bsphack%
  \protected@write\@auxout{}{%
    \string\newacro{#1}[#2]{\AC@uppercase@write #3}%
  }\@esphack%
}%
\def\AC@@acro#1[#2]#3{%
  \ifAC@nolist%
  \else%
  \ifAC@printonlyused%
    \expandafter\ifx\csname acused@#1\endcsname\AC@used%
       \item[\protect\AC@hypertarget{#1}{\acsfont{#2}}] #3%
          \ifAC@withpage%
            \expandafter\ifx\csname r@acro:#1\endcsname\relax%
               \PackageInfo{acronym}{%
                 Acronym #1 used in text but not spelled out in
                 full in text}%
            \else%
               \dotfill\pageref{acro:#1}%
            \fi\\%
          \fi%
    \fi%
 \else%
    \item[\protect\AC@hypertarget{#1}{\acsfont{#2}}] #3%
 \fi%
 \fi%
 \begingroup
    \def\acroextra##1{}%
    \@bsphack
    \protected@write\@auxout{}%
       {\string\newacro{#1}[\string\AC@hyperlink{#1}{#2}]{\AC@uppercase@write #3}}%
    \@esphack
  \endgroup}

\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother




==> etoel.tex <==
From the worst-case execution latencies $TL_{t_i}$ of all the tasks $t_i,\ \forall i$ and the worst-case communication latencies $CL_{m_j}$ of all messages $m_j,\ \forall j$, the worst-case latency of each path in the task graph can be computed as follows
\begin{equation}
L_{path} = \sum_{\forall i\in path} TL_{t_i} + \sum_{\forall j\in path} CL_{m_j}
\label{eqn:pathlat}
\end{equation}
\noindent This is computed for all the paths that exist in the task graph.
Finally, the path with the maximum latency gives the worst-case end-to-end latency of the application.

==> figures/graphs/aspdac_graphs.tikz.tex <==

\tikzstyle{task}=[circle, drop shadow, draw= black, top color=gray!20, bottom color=gray!10, minimum width=0.25cm]
\tikzstyle{comm}=[circle, drop shadow, draw= black, top color=white, bottom color=white, minimum width=0.1cm, inner sep=0.2mm]
\tikzstyle{myarrow} =[->,draw=darkgray,darkgray, line width=0.8pt,>=stealth]


\tikzstyle{cluster} =[rectangle, inner sep=0.2cm, fill=white, drop shadow, rounded corners, draw=darkgray, line width=0.8pt, minimum height=1.0cm, text centered]

\definecolor{myblue1}{RGB}{192,215,228}
\definecolor{myblue2}{RGB}{170,201,219}
\tikzstyle{colorBlue}=[top color=myblue1, bottom color=myblue2]



\newcommand{\drawTaskGraph}{
\scriptsize
   \node[task] at (0,0) (t1) {$t_0$};
   \node[task] at (-1.5,-1.75) (t2) {$t_1$};
   \node[task] at (1.5,-1.75) (t3) {$t_2$};
   \node[task] at (0,-3.5) (t4) {$t_3$};

   % t1 to t2
   \draw[draw=none] (t1)  to node[comm] (c12) {\scriptsize $m_0$} (t2);
   \draw[myarrow] (t1)  edge[->] (c12);
   \draw[myarrow] (c12)  edge[->] (t2);
   
   % t1 to t3
   \draw[draw=none] (t1)  to node[comm] (c13) {\scriptsize $m_1$} (t3);
   \draw[myarrow] (t1)  edge[->] (c13);
   \draw[myarrow] (c13)  edge[->] (t3);
   
   % t2 to t4
   \draw[draw=none] (t2)  to node[comm] (c24) {\scriptsize $m_2$} (t4);
   \draw[myarrow] (t2)  edge[->] (c24);
   \draw[myarrow] (c24)  edge[->] (t4);
   
   % t3 to t4
   \draw[draw=none] (t3)  to node[comm] (c34) {\scriptsize $m_3$} (t4);
   \draw[myarrow] (t3)  edge[->] (c34);
   \draw[myarrow] (c34)  edge[->] (t4);	
	
}


\newcommand{\drawConstraintGraph}{
\small
   %%%%%%%%%
   %% LABELS Cluster
   \node[text width=3.9cm] at (6.5,-0.5) (clusterlabel) {\textbf{task cluster 
$\taskcluster$}:\\$type(\taskcluster)$\\$load(\taskcluster)$\\$\Kmax(\taskcluster)$\\$\prios$};

   %
   \draw[] (1.4,0.1) -- (clusterlabel);
   
   \node[text width=3.9cm] at (6.5,-2.3) (messagelabel) {\textbf{message cluster 
$\commchannel$}:\\$hop(\commchannel)$\\$\SL(\commchannel)$};
   %
   \draw[] (1.4,-1.25) -- (messagelabel);
   
   %%%%%%%%%
   %% Clusters
   \draw[drop shadow, fill=white] (1.2,0) ellipse (2.5cm and 0.7cm);
   \draw[drop shadow, fill=white] (1.2,-2.5) ellipse (2.5cm and 0.7cm);
    \draw[drop shadow, fill=white] (1.2,-1.25) ellipse (1.8cm and 0.4cm);
    %%%%%%%%
   %% Tasks
   \node[task] at (0,0) (t1) {$t_0$};
   \node[task] at (2.5,0) (t2) {$t_1$};
   \node[task] at (0.0,-2.5) (t3) {$t_2$};
   \node[task] at (2.5,-2.5) (t4) {$t_3$};

   
   
   % t1 to t2
   \draw[draw=none] (t1)  to node[comm] (c12) {\scriptsize $m_0$} (t2);
   \draw[myarrow] (t1)  edge[->] (c12);
   \draw[myarrow] (c12)  edge[->] (t2);
   
   % t1 to t3
   \node[comm] at(0.5,-1.25) (c13) {\scriptsize $m_1$};
%    \draw[draw=none] (t1)  to node[comm] (c13) {\scriptsize $m_2$} (t3);
   \draw[myarrow] (t1)  edge[->] (c13);
   \draw[myarrow] (c13)  edge[->] (t3);
   
   % t2 to t4
 %  \node[comm] (c24) at (1,1) {\scriptsize $m_3$}
    \node[comm] at(2,-1.25) (c24) {\scriptsize $m_2$};
  % \draw[draw=none] (t2)  to node[comm] (c24)  {\scriptsize $m_3$} (t4);
   \draw[myarrow] (t2)  edge[->] (c24);
   \draw[myarrow] (c24)  edge[->] (t4);
   
   % t3 to t4
   \draw[draw=none] (t3)  to node[comm] (c34) {\scriptsize $m_3$} (t4);
   \draw[myarrow] (t3)  edge[->] (c34);
   \draw[myarrow] (c34)  edge[->] (t4);	
   
   %%%%%%%%%
   %% LABELS Tasks
  % \node[text width=1.75cm] at (4.8,-2.5) (tasklabel) {\textbf{task $\task$}:\\$\wcet$};
   %
%   \draw[] (t4) -- (tasklabel);
   

}


==> figures/graphs/aspdac_scheduling.tikz.tex <==

\tikzstyle{task}=[circle, drop shadow, draw= black, top color=gray!20, bottom color=gray!10, minimum width=0.25cm]
\tikzstyle{comm}=[circle, drop shadow, draw= black, top color=white, bottom color=white, minimum width=0.1cm, inner sep=0.2mm]
\tikzstyle{myarrow} =[->,draw=darkgray,darkgray, line width=0.8pt,>=stealth]


\tikzstyle{cluster} =[rectangle, inner sep=0.2cm, fill=white, drop shadow, rounded corners, draw=darkgray, line width=0.8pt, minimum height=1.0cm, text centered]

\definecolor{myblue1}{RGB}{192,215,228}
\definecolor{myblue2}{RGB}{170,201,219}
\tikzstyle{colorBlue}=[top color=myblue1, bottom color=myblue2]

\tikzstyle{task1}=[draw=gray!60!black, fill=gray!40, pattern=north east lines, pattern color=gray!60,]
\tikzstyle{task2}=[draw=gray!60!black, fill=gray!40, pattern=north east lines, pattern color=gray!60,]
\tikzstyle{task3}=[draw=orange!80!black, fill=orange!40]
\tikzstyle{task3os}=[draw=orange!80!black, fill=orange!10]

\newcommand{\drawScheduling}{

  

  \draw[task1] (0,0) rectangle node[] {$t^\prime$} (1,0.75);
  \draw[task2] (1,0) rectangle node[] {$t^{\prime\prime}$} (2,0.75);
  \draw[task3] (2,0) rectangle node[] {$t_i$} (3,0.75);
  \draw[task1] (3,0) rectangle node[] {$t^\prime$} (4,0.75);
  \draw[task2] (4,0) rectangle node[] {$t^{\prime\prime}$} (5,0.75);
  \draw[task3] (5,0) rectangle node[] {$t_i$} (6,0.75);
  \draw[task1] (6,0) rectangle node[] {$t^\prime$} (7,0.75);
  \draw[task2] (7,0) rectangle node[] {$t^{\prime\prime}$} (8,0.75);
  \draw[task3] (8,0) rectangle node[] {$t_i$} (8.4,0.75);
  
  \foreach \x in {0,...,9}
  {
    \draw[draw=gray, line width=1pt] (\x,0) -- (\x,1);
  }
  
  \draw[myarrow] (-0.4,0) to (9.4,0);
  
  \draw[myarrow,<->] (0,-0.75) to (3,-0.75);
  \node[] at (1.5, -1.1) {$K_{max} \cdot SI$};  
  
  \draw[myarrow,<->] (3,-0.75) to (6,-0.75);
  \node[] at (4.5, -1.1) {$K_{max} \cdot SI$};
  
  \draw[myarrow,<->] (6,-0.75) to (9,-0.75);
  \node[] at (7.5, -1.1) {$K_{max} \cdot SI$};
  
  
  \draw[draw=darkgray, dotted] (2,1) -- (1.5,2);
  \draw[draw=darkgray, dotted] (3,1) -- (5.5,2);
  
  
  \draw[task3os] (1.5,2) rectangle node[] {$SI_{os}$} (3.2,3.25);
  \draw[task3] (3.2,2) rectangle node[] {$t_i$} (5.5,3.25);
  \draw[myarrow] (1.2,2) to (5.8,2);
  \draw[draw=gray, line width=1pt] (1.5,2) -- (1.5,3.5);
  \draw[draw=gray, line width=1pt] (5.5,2) -- (5.5,3.5);
}


==> plots/dynamic_vs_fixed_5x5.tex <==
\begin{tikzpicture} 

\begin{axis}[
    x tick label style={ /pgf/number format/1000 sep=}, 
    %%%%%%%
    symbolic x coords={0, 10, 20, 30, 40, 50, 60, 70, 80, 85, 90, 95},
    %%%%%%%
    ylabel = {success rate},
    xlabel = {\ac{NoC} utilization},
    %%%%%%%
    width=\columnwidth,
    height=6.0cm,
    ymin = 0,
    %%%%%%%
    legend style={at={(0.5,-0.25)}, anchor=north,legend columns=-1},    
]


\addplot+[] coordinates {
	(95, 0.125)
	(90, 0.0869565217391304)
	(85, 0.0714285714285714)
	(80, 0.0554323725055432)
	(70, 0.0545886075949367)
	(60, 0.0838150289017341)
	(50, 0.14762741652021)
	(40, 0.28099173553719)
	(30, 0.559322033898305)
	(20, 0.712707182320442)
	(10, 0.92)
	(0, 0.413793103448275)

    };
    
%\addplot+[const plot mark mid]
\addplot+[] coordinates {
	
	(95, 0.0357142857142857)
	(90, 0.0555555555555555)
	(85, 0.0588235294117647)
	(80, 0.0707070707070707)
	(70, 0.0628930817610062)
	(60, 0.0657015590200445)
	(50, 0.0717488789237668)
	(40, 0.131608548931383)
	(30, 0.25)
	(20, 0.644927536231884)
	(10, 0.87037037037037)
	(0, 1)

};


\legend{fixed SL, flexible SL} 

\end{axis} 

\end{tikzpicture}

==> plots/runtime_cdf.tex <==
\begin{figure*}[t]
	\centering
	\subfigure[Execution times successful mappings.]{
\begin{tikzpicture}
\pgfplotstableread{results/executiontime_cdf_success.dat}{\pistonkinetics}
\begin{axis}[minor tick num=1,
width = 0.47\linewidth,
height = 6 cm,
xlabel=execution time in ms ,
ymin = 0,
ymax = 105,
ylabel = \ac{CDF} in  \%, 
legend style={legend pos=south east},
xmin = -250,
xmax = 2400,
 xticklabels={,0,500,,2500,3000},
 %xtick={0,500,1000,1500,2000},
 ytick={0,25,50,75,95},
extra x ticks={1000}, extra x tick style={grid=major, tick label style={xshift=0cm,yshift=.30cm}},
extra x tick labels={\color{black}{/\!\!\!/}},
 minor ytick={100},
grid=both,
minor grid style={dotted},
legend style={legend pos=south east},
]
\draw[line width=1pt,dotted] (\pgfkeysvalueof{/pgfplots/xmin},95) -| (437,\pgfkeysvalueof{/pgfplots/ymin});
%\addplot [black,very thick] table [x={class}, y={Sharing_order}] {\pistonkinetics};
\addplot [red,very thick, restrict x to domain=0:1000] table [x expr=\thisrowno{0}, y expr=\thisrowno{1}*100] {\pistonkinetics};
%\draw [red, thick] (axis cs:1000,-.15) -- (axis cs:1000,.15);
  %\draw[black] {(axis cs:1000,80) -- (axis cs:1000,0)};
  \draw[gray] decorate [decoration={zigzag}] {(axis cs:990,\pgfkeysvalueof{/pgfplots/ymax}) -- (axis cs:990,0)};
	  \draw[gray] decorate [decoration={zigzag}] {(axis cs:1010,\pgfkeysvalueof{/pgfplots/ymax}) -- (axis cs:1010,0)};
\addplot [red,very thick, restrict x to domain=1000:3400] table [x expr=\thisrowno{0}-1000, y expr=\thisrowno{1}*100] {\pistonkinetics};
	  \draw[black] (axis cs: 2205		,100) -- node[left]{\scriptsize{max  exec. time}} (axis cs: 2205,0);
%\addplot [dashdotdotted,blue,very thick] table [x expr=\thisrowno{0}*100, y expr=\thisrowno{3}*100] {\pistonkinetics}; %
%\legend{\textbf{ti}, \textbf{spi}}
\end{axis}
% \pgfplotstableread{results/ReliabilityExperimentPareto_time_new.dat}{\pistonkinetics}
% \begin{axis}[minor tick num=1,width = 0.32\textwidth,
%   hide x axis,    axis y line*=right, ylabel = Execution time
% ]
% \addplot [black,very thick] table [x={class}, y={Sharing_order}] {\pistonkinetics};
% \addplot [red,very thick] table [x expr=\thisrowno{0}*100, y={Sharing_non_order}] {\pistonkinetics};
% \addplot [dashdotdotted,blue,very thick] table [x expr=\thisrowno{0}*100, y={Exclusive}] {\pistonkinetics}; %
% \legend{\textbf{ti}, \textbf{spi}} 
% \end{axis}
\end{tikzpicture}
\label{fig:execsuc}
}
\subfigure[Execution times of failed mappings.]{
\begin{tikzpicture}
\pgfplotstableread{results/executiontime_cdf_fail.dat}{\pistonkinetics}
\begin{axis}[minor tick num=1,
width = 0.49\linewidth,
height = 6 cm,
xlabel=execution time in ms ,
ymin = 0,
ymax = 105,
ylabel = \ac{CDF} in  \%, 
legend style={legend pos=south east},
grid=both,
xmin = -250,
xmax = 2400,
 xticklabels={,0,500,,7500,8000},
 %xtick={0,500,1000,1500,2000},
 ytick={0,25,50,75,95},
extra x ticks={1000}, extra x tick style={grid=major, tick label style={xshift=0cm,yshift=.30cm}},
extra x tick labels={\color{black}{/\!\!\!/}},
minor ytick={100},
grid=both,
minor grid style={dotted}
]
\draw[line width=1pt,dotted]  (\pgfkeysvalueof{/pgfplots/xmin},95) -| (506,\pgfkeysvalueof{/pgfplots/ymin});
%\addplot [black,very thick] table [x={class}, y={Sharing_order}] {\pistonkinetics};
\addplot [red,very thick, restrict x to domain=0:1000] table [x expr=\thisrowno{0}, y expr=\thisrowno{1}*100] {\pistonkinetics};
  \draw[gray] decorate [decoration={zigzag}] {(axis cs:990,\pgfkeysvalueof{/pgfplots/ymax}) -- (axis cs:990,0)};
	  \draw[gray]  decorate [decoration={zigzag}] {(axis cs:1010,\pgfkeysvalueof{/pgfplots/ymax}) -- (axis cs:1010,0)};
\addplot [red,very thick, restrict x to domain=1000:3400] table [x expr=\thisrowno{0}-6000,y expr=\thisrowno{1}*100] {\pistonkinetics};
	  \draw[black] (axis cs: 2112	,100) -- node[left]{\scriptsize{max  exec. time}} (axis cs: 2112,0);
%\addplot [dashdotdotted,blue,very thick] table [x expr=\thisrowno{0}*100, y expr=\thisrowno{3}*100] {\pistonkinetics}; %
%\legend{\textbf{ti}, \textbf{spi}}
\end{axis}
% \pgfplotstableread{results/ReliabilityExperimentPareto_time_new.dat}{\pistonkinetics}
% \begin{axis}[minor tick num=1,width = 0.32\textwidth,
%   hide x axis,    axis y line*=right, ylabel = Execution time
% ]
% \addplot [black,very thick] table [x={class}, y={Sharing_order}] {\pistonkinetics};
% \addplot [red,very thick] table [x expr=\thisrowno{0}*100, y={Sharing_non_order}] {\pistonkinetics};
% \addplot [dashdotdotted,blue,very thick] table [x expr=\thisrowno{0}*100, y={Exclusive}] {\pistonkinetics}; %
% \legend{\textbf{ti}, \textbf{spi}} 
% \end{axis}
\end{tikzpicture}
\label{fig:execfail}
}
\caption{CDF of backtracking algorithm execution times.  Note the discontinuity in the x-axis in both plots. The values between 1,000 and 2,000 in~(a) and 1,000 and 7,000 in in (b) are left out as the slope is marginal there.  The maximal needed execution time is denoted on the right of each plot with a vertical line. }
\label{fig:exectimes}
\end{figure*}

==> runtime.tex <==
\begin{color}{red}
  Generally, application mapping is performed by binding tasks to \acp{PE}, and performing their scheduling and the routing of messages over the \ac{NoC}. 
  The number of possible mappings grows exponentially with the number of tasks, and finding feasible and optimal mappings is NP-complete. 
  The idea behind hybrid application mapping is to perform this complex task at design time to determine a set of non-dominated operating points by applying \ac{DSE} techniques, e.g., based on \acp{EA} \cite{WGWGT14,2parma:2012}. 
  Any mapping generated by \ac{DSE} can be represented by a constraint graph $\Gconstraint$ for handing over the \ac{DSE} result to the run-time management. 
  Fig.~\ref{fig:cluster graphs} gives an example. 
  Vertices are given by $\Vconstraint = \taskclusters \cup \commchannels$. 
\end{color}
% 
% We realize the embedding of applications with predictable execution time guarantees through a combination of design time analysis and
% run-time embedding.
% For this purpose, we perform a \ac{DSE} with the afore detailed analysis of
% the worst-case end-to-end latency.
% As an intermediate representation for handing over the results of the \ac{DSE}, we use a constraint graph $\Gconstraint$, where vertices are
% given by $\Vconstraint = \taskclusters \cup \commchannels$.
%In the following 
A \textit{task cluster} $\taskcluster \in \taskclusters$ represents a set of tasks
which are mapped to the same \ac{PE} of the type $type(\taskcluster) \in \RES$ and induces together the load
$load(c)$ on this \ac{PE}:
\begin{equation}
load(c)=\sum_{\forall \task \in \taskcluster } 
\frac{ \left\lceil \dfrac{\wcet}{\SI} \right\rceil \times (\SI+\SIos)}
     {\period}
\end{equation}
$\commchannel \in \commchannels$ denotes a \textsl{message cluster} which is a set of all messages which share the preceding and
succeeding task cluster.
The goal of the run-time embedding is to map $\Vconstraint$ onto the architecture $\Garch$.
Here, each task cluster has to be assigned to a \ac{PE}: $\map_\taskcluster: \taskclusters \rightarrow \pes$ and the message cluster needs
to be mapped onto a route of links by the routing  $\map_\commchannel: \commchannels \rightarrow 2^{\links}$.
To conduct this mapping, based upon the analysis performed during design time, several information about this analysis have to
be annotated.
This holds for the maximum number of additional task $K_{max}$ as well as for the service interval $\SI$.
In addition the priorities $\prios$ of the task are annotated.
% An example such a constraint graph is given in Fig. \ref{fig:cluster graphs}. 
%and priority information ofpredecessors $\preds$ (negative if external) 
%The function $\predf$ is defined as follows:
% \begin{equation}
% \predf(t)=
%    \begin{cases}
%     \prio(pred(t)), &\text{if $pred(t)$ local}\\
%     -1, &\text{otherwise}.    
%   \end{cases}
% \end{equation}

\begin{figure}[t]
 \centering
 \input{figures/graphs/aspdac_graphs.tikz.tex}
    \begin{tikzpicture}
    \drawConstraintGraph
    \end{tikzpicture}
  \caption{Representation of task cluster graph of an explored mapping containing two task clusters and one message cluster  with
annotated constraint information.}
 \label{fig:cluster graphs}
\end{figure}

To find a run-time embedding which corresponds to design-time analysis certain constraints need to be fulfilled.
Therefore, we formulate the problem of run-time binding as a \acfi{CSP} based on the constraint graph.
The goal is here to find a variable assignment that does not violate the following constraints.
Let assume that the task cluster $c_1$ should be mapped onto the \ac{PE} $\targetpe$, the succeeding message cluster $\commchannel$
($\commchannel=succ_c(c_1)$) to the route $\links_m$ and the succeeding task cluster $c_2$ ($c_2=succ_c(\commchannel)$) onto
the \ac{PE} $\targetpetwo$.
Further, there are already previously mapped task clusters $\taskclusters^\prime$ and message clusters $\commchannels^\prime$ in the system.
%($\map_{\taskcluster}(\taskcluster)=\targetpe$) 
First, constraints concerning message clusters $\commchannel \in \commchannels$ are formulated:

\begin{enumerate}[label=\textbf{C.\arabic*}]
   \item The maximal hop count of $\commchannel$ must not exceed the
hop count of the mapped message cluster:
	\begin{align}
	\hop\left( \pe_1, \pe_2 \right) \le hop(\commchannel)        
   \end{align}
   \label{const:hops}
   \item $\SL(\commchannel)$ and the accumulated  $\SL(\commchannel\prime)$ of already mapped messages $\SL_l$ on a link $\link$ need to be less or equal than
$\SLmax$ on every link $\link$ on the route $\links_\commchannel$:
\begin{align}
	 \SL(\commchannel) +\sum_{\overset{\commchannel^\prime \in \commchannels^\prime:}{l \in \map_\commchannel(\commchannel^\prime)}}
\SL(\commchannel^\prime)  \le \SLmax, \forall l \in \links_\commchannel     
\end{align}
%After a successful mapping $\SL_l$ is updated to $\SL_l^{\prime}$:
%\begin{align}
%\SL_l^{\prime} = \SL(\commchannel) + \SL_l 
%\end{align}
\end{enumerate}
Second, constraints for mapping $\taskcluster \in \taskclusters$ to the selected target $\targetpe$ have to be fulfilled:
\begin{enumerate}[label=\textbf{C.\arabic*}]
  \setcounter{enumi}{2}
 \item The type of $\targetpe$  has to be the same as $type(\taskcluster)$: \label{const:type}
\begin{align}
    type(\taskcluster)=\rtype(\targetpe)
\end{align}
 \item The load $load(\taskcluster)$ needs to be smaller than the still available load on $\targetpe$: \label{const:load}
\begin{align}
    load(\taskcluster) \le 1 - \sum_{\overset{\taskcluster^\prime \in \taskclusters^\prime:}{\targetpe =
\map_\taskcluster(\taskcluster^\prime)}} load(\taskcluster^\prime)
\end{align}
% After the mapping a new task cluster $\taskcluster^{\prime \prime} = \taskcluster^\prime \cup \taskcluster$ is created and the load is set correspondingly:
% \begin{align}
%    load(\taskcluster^{\prime \prime} ) =  load(\taskcluster) + load(\taskcluster^\prime)
% \end{align}
% \item The number of mapped tasks on $\pe_c$ need to be less or equal than $K_{max}$.\label{const:kmax}
% \item The number of newly mapped tasks to $\pe_c$ together with the already mapped tasks $K$ may not exceed any $K_{max}$ of already mapped tasks.\label{const:k}
% \item Let the number of tasks mapped on $\targetpe$ be $K(\taskcluster^\prime)$, the number of additional tasks allowed on $\targetpe$ be
%$K_{max}(\taskcluster^\prime)$ and the number of tasks in $c$ be $K(\taskcluster)$ then it must be always assured that:
 \item The number of already mapped tasks and the number of tasks in the task cluster $K(\taskcluster)$ must not
exceed any number of maximal tasks which was employed during performance analysis:
\begin{align}
\underset{\taskcluster^\prime \in \taskclusters^\prime: \targetpe =
\map_\taskcluster(\taskcluster^\prime)}{min} & \left\{K(\taskcluster)+K_{max}(\taskcluster),
K(\taskcluster^\prime)+K_{max}(\taskcluster^\prime) \right\} \geq \\[-0.6cm] \nonumber
 &K(\taskcluster) + \sum_{\overset{\taskcluster^\prime \in \taskclusters^\prime:}{\targetpe =
\map_\taskcluster(\taskcluster^\prime)}} K(\taskcluster^\prime)
\end{align}
\vspace{-0.5cm}
% After the mapping the new parameters are set:
% \begin{align}
% K(\taskcluster^{\prime \prime}) &= K(\taskcluster^\prime) + K(\taskcluster) \\
% K_{max}(\taskcluster^{\prime \prime} ) &= min \left\{ K_{max}(\taskcluster)-K(\taskcluster^\prime), K_{max}(\taskcluster^\prime) - K(\taskcluster) \right\}
% \end{align}
\label{const:k}
% \item $TL_{t}$ of any tasks $\task \in \taskcluster$ may not be increased through the mapping of $\taskcluster$.
\end{enumerate}
\begin{figure}[t]
	\centering
		\includegraphics[width=1.00\columnwidth]{figures/ne_mapping.pdf}
	\caption{Example of a mapping of a task cluster $c$ to $\targetpe$. The number of tasks in $c$ is $K(c)=2$ and the number of
additional tasks $K_{max}(c)=2$. The number of tasks already present at  $\targetpe$ is $K(c^\prime)=2$ and $K_{max}(c^\prime)=2$. After the
mapping $c^{\prime\prime}$ is created and $K(c^{\prime\prime})=4$ and $K_{max}(c^{\prime\prime})=0$.  The priorities of the tasks are
annotated in circles. After the mapping the priorities of $c$ are updated to \textcircled{3} and \textcircled{5} in order to keep the
priorities unique.}
		\label{fig:new_mapping}
\end{figure}



In case of a spatial isolation only the \ref{const:type}~constraint for
$\taskcluster$ and the absence of other tasks on $\targetpe$ ($load(\taskcluster^\prime)=0$) would be sufficient to guarantee the worst-case
execution latency (see Eq. \eqref{eqn:tl}) as only tasks
of one application could be mapped together onto a \ac{PE}.
When applying temporal isolation as concept also the other aforementioned constraints need to hold.
%If the constraints~\ref{const:kmax} and \ref{const:k} are fulfilled $TL_{t}$ can be checked.
%If the timing analysis of the task cluster $c$ was carried out with different
%parameters, i.e. $\SI$, than which are present at $\targetpe$, then a part
%of the calculation of the worst-case execution latency has to be re-calculated.
%Let assume that the worst-case execution latency of the newly mapped task
%together with the already mapped tasks and the $\SI$ present at $\targetpe$
%is $TL_{t}^{\prime}$=$TL_{exec,t}^{\prime}+TL_{inter,t}^{\prime}$.
%For a system wide fixed $\SI$ and $\SIos$ only $TL_{inter,t}$
%and $TL_{inter,t}^{\prime}$ has to be examined during run time.
%With the information of $\prios$ and $\preds$ Eqn.~(\ref{eqn:tinterb}) can be
%re-calculated.
%If $TL_{t}^{\prime} \le TL_{t}$ then $c$ can safely be mapped to $\targetpe$ without worsening of the worst-case execution latency.
% If $\SI(c)$ differs from the current $\SI$ of $\pe$ additionally $TL_{exec,t}$ and $TL_{exec,t}^{\prime}$ need to be calculated with both
%service intervals.
If all constraints are fulfilled and the priority ranges of $c$ and $c^\prime$ overlap, the priorities of $c^\prime$ are shifted after
mapping to keep them unique on the \ac{PE}. 
An example of the priority assignment and the constraint~\ref{const:k} and can be found in Fig.~\ref{fig:new_mapping}.

To find an embedding which satisfies all the introduced constraints and to solve the \ac{CSP} we use a backtracking algorithm like shown in
Algo.~\ref{algo:backtracking}. 
This algorithm starts with $\mathcal{A}=\emptyset$ and then searches recursively for a valid variable assignment for $\mathcal{A}$.  
In line~\ref{algo:BT:select} the next variable to check is selected and in line~\ref{algo:BT:domain} the domain $D_c$ with all \acp{PE}
which fulfill \ref{const:hops} and \ref{const:type} is created.
In the lines~\ref{algo:BT:testStart}~to~\ref{algo:BT:testEnd} the remaining constraints are checked.


 \begin{algorithm}[t]
 \label{algo:backtracking}
     {\tt backtrack}($\mathcal{A} $, $\Gconstraints$, $\Garchs$)\\
     \If{($\mathcal{A} $ is complete)\label{algo:BT:cond1}}{
       \textbf{return} $\mathcal{A} $\;
     }
     $c$ = selectNextUnassignedVariable($T_C$)\;\label{algo:BT:select}
     $D_c$ = doForwardChecking($c$, $\Gconstraints$,$\Garchs$)\;\label{algo:BT:domain}
 
     \For{\textbf{each} $\left( \targetpe \in D_c \right)$\label{algo:BT:testStart}} {
 	\If{$\targetpe$ enables feasible binding and routing $L_\commchannel$}{
 	    $\mathcal{A} ^\prime$ = {\tt backtrack}($\mathcal{A} \cup \langle c, \targetpe, L_\commchannel \rangle$, $\Gconstraints$,
$\Garchs$)\;\label{algo:BT:recursion}
 
 	    \If{($\mathcal{A} ^\prime \ne \emptyset$)}{
 	      \textbf{return} $\mathcal{A} ^\prime$\;
 	    }\label{algo:BT:testEnd}
 	}
     }
     
      \textbf{return} $\emptyset$\;
 \caption{Backtracking algorithm for finding a feasible constraint graph embedding.}
 \end{algorithm}

